Patterns of Patient and Caregiver Mutual Support Connections in an Online Health Community

Online health communities offer the promise of support benefits to users, in particular because these communities enable users to find peers with similar experiences. Building mutually supportive connections between peers is a key motivation for using online health communities. However, a user's role in a community may influence the formation of peer connections. In this work, we study patterns of peer connections between two structural health roles: patient and non-professional caregiver. We examine user behavior in an online health community where finding peers is not explicitly supported. This context lets us use social network analysis methods to explore the growth of such connections in the wild and identify users' peer communication preferences. We investigated how connections between peers were initiated, finding that initiations are more likely between two authors who have the same role and who are close within the broader communication network. Relationships are also more likely to form and be more interactive when authors have the same role. Our results have implications for the design of systems supporting peer communication, e.g. peer-to-peer recommendation systems.

==> double-fig.tex <==
\begin{figure}
\centering
\begin{subfigure}[t]{0.5\textwidth}
  \includegraphics[height=2.74in]{figures/collab_authorship.pdf}
\caption{Thresholds in the distribution where 15.5\% of \\ sites are independently authored by patients, \\45.1\% are collaboratively edited, and 39.4\% are \\independently authored by non-patients.}
\label{fig:counts}
\end{subfigure}%
\begin{subfigure}[t]{0.5\textwidth}
  \includegraphics[height=2.74in]{figures/majority_authorship.pdf}
\caption{Threshold where 63.5\% of sites are majority non-patient authored (i.e. >50\% of updates classified as non-patient authored).}
\label{fig:freq}
\end{subfigure}
\caption{Distribution of sites by proportion of patient-authored journal updates. (Same distribution, both imgs.)}
\label{fig:ML_authorship}
\end{figure}
